Teaching Divisibility and Binomials with Coq

The goal of this contribution is to provide worksheets in Coq for students to learn about divisibility and binomials. These basic topics are a good case study as they are widely taught in the early academic years (or before in France). We present here our technical and pedagogical choices, the numerous exercises we developed and a small experiment we conducted on two students. As expected, it required additional Coq material such as other lemmas and dedicated tactics. The worksheets are freely available and flexible in several ways.

==> eptcsdata.tex <==
\providecommand{\firstpage}{124}
\providecommand{\publicationstatus}{J. Narboux, W. Neuper and P. Quaresma (Eds.): Theorem Proving\\ Components for Educational Software 2024 (ThEdu'24)\\
EPTCS 419, 2025, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.419.8}{10.4204/EPTCS.419.8}}
\pdfoutput=1

